BenLLMEval: A Comprehensive Evaluation into the Potentials and Pitfalls of Large Language Models on Bengali NLP

Large Language Models (LLMs) have emerged as one of the most important breakthroughs in NLP for their impressive skills in language generation and other language-specific tasks. Though LLMs have been evaluated in various tasks, mostly in English, they have not yet undergone thorough evaluation in under-resourced languages such as Bengali (Bangla). To this end, this paper introduces BenLLM-Eval, which consists of a comprehensive evaluation of LLMs to benchmark their performance in the Bengali language that has modest resources. In this regard, we select various important and diverse Bengali NLP tasks, such as text summarization, question answering, paraphrasing, natural language inference, transliteration, text classification, and sentiment analysis for zero-shot evaluation of popular LLMs, namely, GPT-3.5, LLaMA-2-13b-chat, and Claude-2. Our experimental results demonstrate that while in some Bengali NLP tasks, zero-shot LLMs could achieve performance on par, or even better than current SOTA fine-tuned models; in most tasks, their performance is quite poor (with the performance of open-source LLMs like LLaMA-2-13b-chat being significantly bad) in comparison to the current SOTA results. Therefore, it calls for further efforts to develop a better understanding of LLMs in modest-resourced languages like Bengali.

==> not_needed.tex <==


\subsection{Error Analysis}
\label{sec:error_analysis}
We found some interesting cases where LLMs failed to generate coherent responses given the input prompt. We discuss these cases for the overall best-performing LLM, ChatGPT, in the following:\\
%\\ \subsubsection{Generative Tasks}\label{sec:generative}\\
%The error cases for generative tasks like abstractive summarization, question answering, and paraphrasing is discussed in this section.\\ 

\subsubsection{Text Summarization}
\label{sec:as}

In the summarization task, we notice that ChatGPT's responses are highly inconsistent. While ChatGPT occasionally recognizes the context and provides a good summary of the key points, it frequently misses these details in the reference text and overstuffs the response. One example can be demonstrated as follows: \\
\textbf{Prompt:} Please provide an one-sentence summary of the following Bangla text input. The input will be a long Bangla paragraph, the output should be a short Bangla paragraph summarizing only the vital information of the input text in one sentence. Please make sure that the output contains the most essential statistical data.
Note: Please do not provide anything other than the summarized Bangla output. \\
\textbf{Input:} \textbengali{মানসুর আব্বাস প্রধানমন্ত্রী বা তার প্রতিপক্ষ - কেউই আসলে ক্ষমতায় যাবার মতো নিরঙ্কুশ সংখ্যাগরিষ্ঠতা পাননি। আর এর মধ্যেই কিংমেকার হয়ে উঠেছে রাম (Raam) নামে একটি ইসলামপন্থী আরব দল (ইউনাইটেড আরব লিস্ট হিসেবেও দলটি পরিচিত)। এবারের নির্বাচনে ...}(\textit{long text})\\
\textbf{Expected Response:} \textbengali{গত দু বছরের মধ্যে চতুর্থবারের মতো একই সমস্যা হচ্ছে ইসরায়েলে- নির্বাচনের পর সংখ্যাগরিষ্ঠতা পেয়েও ক্ষমতায় থাকার জন্য প্রয়োজনীয় আসনের জন্য হাহাকার করতে হচ্ছে প্রধানমন্ত্রী বেনিয়ামিন নেতানিয়াহুকে।}\\
\textbf{ChatGPT Response:} \textbengali{ মানসুর আব্বাস নেতৃত্বের রাম দল ইসরায়েলের পার্লামেন্টে পাঁচটি আসন জিতেছে এবং এদের কিংমেকার হয়ে উঠার পথ তৈরি করেছে, তিনি ইউনাইটেড আরব লিস্টের নেতা হিসেবে পরিচিত এবং ইসরায়েলে আরব রাজনীতি প্রায় নব্বই লাখ মানুষের মধ্যে উনিশ লাখের মতো আরব আছেন যারা ১৯৪৮ সালে ইসরায়েলের সীমানায় থেকে গিয়েছিলেন।}\\
In the aforementioned example, ChatGPT fails to highlight the most crucial information from the input and saturates the output with superfluous texts.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[h]
\centering

\begin{tabular}{lllll}
\hline
                            &  & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ \hline
\textbf{Before Translation} &  & 0.41         & 0.14         & 0.34         \\ \hline
\textbf{After Translation}  &  & 4.69         & 0.61         & 3.61         \\ \hline
\end{tabular}%
\caption{Performance of Llama-2-13b-chat on Summarization Before and After Translation }
\label{tab:llama_summarization}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Question Answering}
\label{sec:QA}

In the Question Answering task, ChatGPT is given instructions to provide responses based on the given context. However, there are instances where ChatGPT deviates from the context and attempts to answer using information from its general knowledge, resulting in a mismatch with the gold label. While this problem occurred only in a limited number of cases, the authors were unable to independently verify the accuracy of the responses in these instances, leading to their classification as incorrect answers.\\
\textbf{Prompt:} Please provide an answer to the input Bangla question based on the given Bangla context. The input will contain a Bangla question followed by a context. The output should be the answer in Bangla based on the context. Note: Please do not provide anything other than the Bangla answer to the question.\\
\textbf{Context:} \textbengali {নেপালের রাজধানী কাঠমুন্ডুর উপত্যকায় প্রাপ্ত নিওলিথিক যুগের বেশকিছু উপাদান এটিই নির্দেশ করে যে হিমালয়ান অঞ্চলে প্রায় ৯০০০ বছর থেকে মানুষ বসবাস করছে। এটি প্রতিষ্ঠিত যে প্রায় ২৫০০ বছর পূর্বে নেপালে তিব্বতী-বার্মীয় জনগোষ্ঠীর বসবাস ছিল। ১৫০০ খৃস্টপূর্বাব্দে ইন্দো ইরানীয় বা আর্য জাতিগোষ্ঠী এই হিমালয়ান উপত্যকায় প্রবেশ করে। ১০০০ খৃস্টপূর্বাব্দের দিকে এই অঞ্চলটিতে বিভিন্ন গোষ্ঠীর জন্য স্বতন্ত্র রাজ্য ও কনফেডারেশন গড়ে উঠে। এরকমই একটি কনফেডারেশন ...}\\
\textbf{Question:} \textbengali{নেপাল কি একটি সার্বভৌম দেশ ?}\\
\textbf{Expected Response: } No Answer.\\
\textbf{ChatGPT Response: } \textbengali{হ্যাঁ, নেপাল একটি সার্বভৌম দেশ।}\\
In this particular instance, ChatGPT provides responses that go beyond the scope of the given context, as the context itself lacks the necessary information to yield the correct answer. Consequently, this deviation from the context leads to a mismatch with the gold label, ultimately resulting in an incorrect response.

\subsubsection{Paraphrasing}
\label{sec:paraphrase}
In some instances, ChatGPT generates paraphrase that completely changes the meaning of the input sentences. For example: \\
\textbf{Input: } \textbengali{আগুনে কোনও হতাহতের খবর পাওয়া যায়নি।} [No injury was reported because of the fire] \\
\textbf{Expected Responses: } [\textbengali{'অগ্নিকাণ্ডে উল্লেখযোগ্য কোন ক্ষয়ক্ষতি হয়নি।', 'অগ্নিকাণ্ডে উল্লেখযোগ্য কোন ক্ষয়ক্ষতি হয়নি।', 'এই অগ্নিকাণ্ডে হতাহতের কোনও খবর মেলেনি।', 'এই অগ্নিকাণ্ডে হতাহতের কোনো খবর পাওয়া যায়নি।', 'অগ্নিকাণ্ডে হতাহতের কোনো খবর পাওয়া যায়নি।', 'অগ্নিকাণ্ডে কারও হতাহতের খবর পাওয়া যায়নি।'}]\\
\textbf{ChatGPT Response:} \textbengali{কোন আপত্তিকর ঘটনা না হওয়ায় আগুনের সম্পর্কে কোন খবর পাওয়া যায়নি।} [There was no news about the fire as there was no untoward incident.]
This is a matter of concern and presents additional evidence that ChatGPT is not currently suitable for serving as a universal problem solver in the Bangla language.


%\paragraph{Classification Tasks}
%\label{sec:txtcls}
%In this section, we discuss about the error cases in the other three tasks that we consider: Natrual Language Inference (NLI), Text Classification, and Sentiment Analysis. 

\subsubsection{Natural Language Inference}
\label{sec:nli}
The confusion matrix obtained by evaluting ChatGPT for the NLI task is demonstrated in Figure \ref{fig:conf_nli}. The matrix reveals that ChatGPT demonstrates high accuracy in predicting the \textit{Contradiction} and \textit{Entailment} labels, but encounters significant challenges in accurately predicting the \textit{Neutral} labels. Approximately 49\% of the misclassifications arise when attempting to predict the \textit{Neutral} class. A thorough manual examination uncovers that ChatGPT often exhibits bias towards expressing a particular opinion polarity (\textit{Contradiction, Entailment}) when dealing with logical relationships in Bangla, and it fails to appropriately recognize and convey neutrality even in cases where it is evident.



% \begin{figure}[h]
% \centering
% \includegraphics[scale = 0.53]{figures/foo.png}
% \caption{Confusion matrix obtained by evaluating ChatGPT for the NLI task on BNLI dataset}
% \label{fig:conf_nli}
% \end{figure}

\begin{figure*}[h]
\centering
\includegraphics[width=\textwidth]{figures/conf combined.png}
\caption{Confusion matrix for (a) ChatGPT on the BNLI dataset, (b) Llama-2-13b-chat on the SentNoB dataset, and (c) Claude-2 on the IndicSentiment dataset.}
\label{fig:comb_conf}
\end{figure*}

\textbf{Prompt:} Please determine the logical relationship between the given hypothesis and premise. The input will consist of two sentences written in the Bangla language. The first sentence represents the premise, while the second sentence represents the hypothesis.  Your task is to determine whether the hypothesis is false (contradiction), true (entailment), or inconclusive (neutral) given the premise. Please output a number indicating the logical relationship between them: 0 for false (contradiction), true (entailment), and 2 for inconclusive (neutral) for neutrality. 
Note: Please avoid providing any additional information beyond the logical relationship. \\
\textbf{Premise:} \textbengali{ঠিক আছে, যেখানে দুই-তিনটা বিমান এক সপ্তাহে এসে পৌছেছে এবং আমি জানতাম না তারা কোথায় যাচ্ছে।} \\
\textbf{Hypothesis:} \textbengali{প্রতি সপ্তাহে একটিরও বেশি বিমান আসে।}\\
\textbf{Expected Response: }1 (Entailment)\\
\textbf{ChatGPT Response: }2 (Neutral) 


\subsubsection{News Article Classification}
\label{sec:newscls}
Our experimental results show that ChatGPT misclassified the category \textit{kolkata} the most, failing to generate the correct response in 503 of the test set's 569 examples (88.4\%). The subsequent category with the highest frequency of misclassification is \textit{national}. ChatGPT was unable to accurately classify this particular category in 95 out of 175 instances, representing a misclassification rate of 54.20\%. On the other hand, ChatGPT effectively identified the category labeled as \textit{entertainment} in 110 out of 130 occurrences, resulting in a success rate of 92.30\%.

\subsubsection{Sentiment Analysis}
\label{sec:senti}
The examples listed in the Table \ref{tab:Sentiment_error}, illustrates the error cases where ChatGPT misclassifies the sentiment of the given input. The first seven examples are from the IndicSentiment test set and the rest of the examples are from the SentNoB dataset. Notably, the \textit{positive} class exhibits the most frequent misclassification in both test sets, suggesting that ChatGPT still has a considerable way to go toward attaining a complete understanding of the Bangla language. In the instances where the class is \textit{neutral}, the examples are mostly simple statement with no sentiment word associated with them (table entry 11, and 12), yet ChatGPT classified them as either \textit{negative} or \textit{positive}. Furthermore, ChatGPT demonstrates difficulties in capturing challenging Bangla sentiment words, i.e., \textbengali{অমায়িক} (\textit{Accommodating} in English), \textbengali{সুবিধা} (\textit{Advantage} in English), \textbengali{আপসহীন} (\textit{Uncompromising} in English) etc (example 2, 8, 13 in Table \ref{tab:Sentiment_error}).\\

\paragraph{Unexpected, out of range response:}
\label{sec:outres}
In the tasks of text classification and sentiment analysis, the prompts are designed to include the target classes in order to identify any unexpected or non-class responses. Based on our experimental findings, we observe that the outputs generated by ChatGPT exhibit outcomes that deviate from the expected range of outputs. \\
%
\textbf{\underline{News Article Classification.}} \\
\textbf{Prompt:} For the Bengali news article given in the input, identify the appropriate section title for the article from the following classes: kolkata, state, sports, national, entertainment, international. Note: Do not output any unnecessary words other than just the section title. The response should be in English language and should be one word.
Input : \textbengali{১০০ দিনের কাজের প্রকল্পের সাফল্য দেখতে রাজ্যে আসছেন কেন্দ্রের প্রতিনিধি। সঙ্গে ১০টি রাজ্যের প্রতিনিধিও। ৯ থেকে ১২ জানুয়ারির মধ্যে পাঁচটি জেলায় রাজ্যের ‘উদ্ভাবনী কাজে’র সাফল্য দেখবেন তাঁরা। ঘটনাচক্রে, পঞ্চায়েত নির্বাচনের আগে এই সফর হতে চলেছে। ফলে প্রশাসনের একাংশের মতে, এই সফর ভোটের আগে শাসকদলের কাছে বড় প্রাপ্তি হতে পারে। বিশেষত, রাজ্যগুলির মধ্যে অধিকাংশই যখন...}(\textit{long text})\\
\textbf{Expected Response:} State \\
\textbf{ChatGPT Response:} Development \\
Our study reveals that ChatGPT, in particular, generated the word \textit{Development}, which deviates from the prompted range of responses. The generated output is considered out of range as the prompt specifically instructs the model to produce text within the given categories of \textit{kolkata}, \textit{state}, \textit{sports}, \textit{national}, \textit{entertainment}, and \textit{international}. In addition, the results of our experiment indicate that ChatGPT produced 12 classes that are outside the target class range, thus demonstrating the model's inability to comply with the specified instructions for this specific task. \\
%

% \begin{figure}[h]
% \centering
% \includegraphics[scale=0.45]{figures/IndicSentResultAnalysisVir.png}
% \caption{Confusion matrix obtained by evaluating Llama-2-13b-chat for the Sentiment Analysis task on IndicSentiment dataset}
% \label{fig:conf_indicsent}
% \end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/SentNoBResultAnalysisVir.png}
% \caption{Confusion matrix obtained by evaluating Llama-2-13b-chat for the Sentiment Analysis task on SentNoB dataset}
% \label{fig:conf_sentnob}
% \end{figure}

\noindent\textbf{\underline{Sentiment Analysis.}} \\
\textbf{Prompt:} For the given Input, is the sentiment in the input positive or negative?
Note: Please do not output anything other than the sentiment. Exclude any word like, Sentiment in the response. \\
Input : \textbengali{স্ট্যান্ড-এ রয়েছে লেভেল ইন্ডিকেটর যা বিল্ট-ইন বাবল ভিউ লেভেল এবং থ্রি-ওয়ে হেড যা ৩৬০ ডিগ্রি ঘোরানো যায়।} \\
\textbf{Expected Response:} Positive \\
\textbf{ChatGPT Response:} Neutral \\
In this instance, although we explicitly prompted ChatGPT to generate output that is either positive or negative, it produced a response that falls outside of the designated range, i.e., \textit{Neutral}. This observation implies that the model may possess certain inherent biases towards sentiment classification among the three widely used categories, namely \textit{positive}, \textit{negative}, and \textit{neutral}. 

Additionally, from the confusion matrix in Figure \ref{FIGURE LABEL}, it is evident that the poor performance of the Llama-2-13b-chat model is attributed to consistent misclassification of the \textbf{negative} class as \textbf{positive} class in the SentNoB dataset. Furthermore, within the dataset, the model misclassified more than 200 instances of both the \textbf{neutral} and \textbf{positive} classes.

%%%%%%%%%%%%%%%%%%%%%%Error Analysis%%%%%%%%%%%%






==> tab_and_app/dataset-prompts.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tab_and_app/lex_translit.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\tiny
\centering
\begin{greybox}
\textbf{Task Description:} Please provide the transliteration in native Bengali script for the input word. 
The input will be a word written in Latin script and the output should be the transliterated Bengali word of the given input. Please note that you are not asked to provide translation of the input word, only provide the Bengali transliteration for the given input. \\

\textbf{Note:} Your response should include only the transliterated word in the native Bengali language. Please do not add any explanation with the output.\\ 

\textbf{Input:} adhunalupto\\

\textbf{ChatGPT Response:} \bengalifont{অধুনালুপ্তো}‌
\end{greybox}
\greyboxcaption{Input prompt and response of ChatGPT for the single-word (lexicon) transliteration on Dakshina dataset.}
\label{prompt:lexicon_translit}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


